The Hijackers Guide To The Galaxy: Off-Path Taking Over Internet Resources

Internet resources form the basic fabric of the digital society. They provide the fundamental platform for digital services and assets, e.g., for critical infrastructures, financial services, government. Whoever controls that fabric effectively controls the digital society. In this work we demonstrate that the current practices of Internet resources management, of IP addresses, domains, certificates and virtual platforms are insecure. Over long periods of time adversaries can maintain control over Internet resources which they do not own and perform stealthy manipulations, leading to devastating attacks. We show that network adversaries can take over and manipulate at least 68% of the assigned IPv4 address space as well as 31% of the top Alexa domains. We demonstrate such attacks by hijacking the accounts associated with the digital resources. For hijacking the accounts we launch off-path DNS cache poisoning attacks, to redirect the password recovery link to the adversarial hosts. We then demonstrate that the adversaries can manipulate the resources associated with these accounts. We find all the tested providers vulnerable to our attacks. We recommend mitigations for blocking the attacks that we present in this work. Nevertheless, the countermeasures cannot solve the fundamental problem - the management of the Internet resources should be revised to ensure that applying transactions cannot be done so easily and stealthily as is currently possible.

==> caches.tex <==
\subsection{RIPE Caches Study}\label{sc:caches}
\subsubsection{RIPE Cache Methodology}
We create accounts for n e-mail addresses hosted in the same domain, in b batches, where
\begin{verbatim}
- b=0 => n=10
- b=1 => n=10
- b=2 => n=30
\end{verbatim}
and batches use their own, separate domain each.

\subsubsection{RIPE Caches Results}
Our nameservers received queries from RIPE resolvers from the following IP addresses:
\begin{verbatim}
- 193.0.19.103
- 193.0.19.113
- 193.0.19.114
\end{verbatim}
Our study found that RIPE resolvers use different caches for records received from Answers and from Referrals, 1 and 3 caches respectively.



==> frag.tex <==

%
 
 
 
\section{Background: IPv4 Packet Fragmentation}\label{sc:ipv4:frag}
In this section we provide background on IP fragmentation and path MTU discovery (PMTUD), as well as background on DNS, DNSSEC, BGP and RPKI. Some of the background on IPv4 packet fragmentation is taken from past publication of the authors. %
\subsection{Maximum Transmission Unit}\label{sc:mtu}
The Maximum Transmission Unit (MTU) is the largest number of bytes that can be transmitted over a link in one datagram. The Path MTU between two end points is limited by the lowest MTU on the path \rfc{791}. When packets exceed the path MTU, they will not be received at the destination. To cope with this, the Internet Protocol (IP) provides the possibility to fragment packets into smaller fragmented packets. Most networks support currently MTU of 1492 bytes \rfc{2516}. According to \rfc{791} the minimum MTU in the Internet is $68$ bytes. The DNS responses typically do not exceed 1500 bytes, unless they contain cryptographic material due to the use of DNSSEC \rfc{4033}, \rfc{4034} and \rfc{4035}. Hence, most DNS responses would not fragment. 

\subsection{ICMP Fragmentation Needed}\label{ssc:icmp} 
To reduce fragmentation load on the routers, \rfc{1191} proposes a mechanism to discover the MTU between two hosts. To do so, hosts make use of the Do Not Fragment (DF) bit in the IP header to instruct the routers along the path to not fragment the packet in case the packet exceeds the MTU of the next hop. Instead, intermediate hosts will discard the packet and issue an \textit{ICMP Destination Unreachable} error message (type 3) to the originator with the code \textit{Fragmentation Needed and DF set} (code 4). %
The information in the ICMP error message is stored by the receiving OS, e.g., 10 minutes by default on Linux 3.13. The ICMP error message can be originated by any Internet node on the path between the sender and the receiver and the receiver of the ICMP error message is not expected to know the IP addresses of the nodes on the path. Hence, we use an off-path attacker to issue an ICMP fragmentation needed packet to the nameserver, indicating that it should reduce the MTU when sending packets to the {\em victim} resolver.



The spoofed ICMP error message does not need to be sent from a spoofed source IP address - ICMP error message can originate from {\em any} node on the path. %
In contrast to ICMP with TCP headers, the OSes typically do not apply any checks on the received ICMP error messages with UDP headers, e.g., Linux 3.13. This is due to the fact that UDP is stateless. Hence, crafting a spoofed ICMP fragmentation needed error message is a simple task.

Figure \ref{fig:icmp} shows an example ICMP fragmentation needed error sent by an attacker at IP {\tt 6.6.6.6} to nameserver at IP {\tt 123.0.0.53} telling the nameserver to reduce the MTU to 100 bytes for all packets it sends to the DNS resolver at {\tt 30.0.0.1} The payload of the ICMP packet is the IP header and the first eight bytes of the original packet (that triggered the ICMP error message). The nameserver stores this information and uses it for limiting the size of IP packets to destination IP ({\tt 30.0.0.1}) and protocol (UDP). We illustrate a first and a second fragment of the original IP packet in Figures \ref{fig:frag1} and \ref{fig:frag2} respectively.

\begin{figure}
  \begin{center}
   \includegraphics[width=0.48\textwidth]{img/pkt_icmp_ptb-crop.pdf}
		\caption{ICMP fragmentation needed packet from attacker at 6.6.6.6 to nameserver at 123.0.0.53 indicating an MTU of 100 bytes for resolver at 30.0.0.1}
		\label{fig:icmp}
  \end{center}
\end{figure}


\subsection{IPv4 Fragmentation and Reassembly}\label{sc:frag:reassemble} Upon arrival to the receiver the fragments of an IP packet are stored in an IP defragmentation cache, by default for 30 seconds. The receiving OS uses the IP ID value in the fragments to identify all the fragments of the same original IP packet (they all have the same IP ID value). Then it uses the offset field to reassemble their payload together. The receiver knows that all the fragments of the original IP packet have arrived by checking that the fragment with the lowest offset has a More Fragments (MF) value of zero.

\begin{figure}[!ht]
  \begin{center}
   \includegraphics[width=0.48\textwidth]{img/pkt_dns_frag1_original-crop.pdf}
		\caption{First fragment sent by the nameserver at 123.0.0.53 to the DNS resolver at 30.0.0.1, assuming MTU of 68 bytes.}
		\label{fig:frag1}
  \end{center}
\end{figure}
%
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.48\textwidth]{img/step1_short-crop.pdf}
    \caption{(Step 1.1 Figure \ref{fig:sequence_overview}) Probing the RIR's DNS resolver for fragment acceptance.}
    \label{fig:step1_dnsprobe}
\end{figure}
%
\subsection{UDP Checksum}\label{sc:udpchecksum}
The method to calculate UDP checksum is defined in \rfc{768}. The UDP checksum is calculated as the 16-bit one's complement sum of the fields in IP header, the UDP header and the UDP payload. The UDP checksum value is stored in the UDP header. Upon receipt of a UDP packet the receiver calculates the UDP checksum (using the same procedure as the sender did) and then compares whether it is the same value as in UDP header. If the value differs - the UDP datagram is discarded.

If the checksum in the second spoofed fragment is not adjusted, when the spoofed second fragment is reassembled with the first real fragment, the overall value of the UDP checksum of both fragments is altered, and will differ from the UDP checksum value in the UDP header. Specifically, the spoofed second fragment contains different records than the real second fragment. Hence, the attacker needs to adjust the UDP checksum of the second fragment such that the computation of the UDP checksum using the payload in both fragments remains similar to the original value of UDP checksum in the UDP header.

The attacker can ensure this as follows: the attacker sends a request to the nameserver and receives a response in two fragments (possibly using the ICMP fragmentation needed packet to enforce fragmentation). The attacker calculates the UDP checksum value of the second fragment, then alters the second fragment and calculates the checksum of the altered second fragment. The difference value in the checksum of both second fragments the attacker needs to add (or remove) by altering two bytes (in even location) in the altered second fragment. This is a simple computation since the attacker knows the original value, and knows what bytes were modified, it can efficiently compute the difference and add (or remove) it to the value of UDP checksum of second fragment.

To adjust the value of two bytes the attacker can either modify two bytes in any record in the second altered fragment, or can add the two bytes at the end, after the EDNS \rfc{6891} record (in this case the DNS software will ignore these two bytes but they will be included in the UDP checksum computation). %


\subsection{IP Identifier (IPID)}\label{sc:ipid} The spoofed second fragment should contain the correct IPID value -- the same value as the original IP packet sent by the nameserver. The attacker must predict this value correctly, otherwise, when the first fragment and the spoofed second fragment have different IPID values, the receiving OS will not reassemble them together. 

Predicting the IPID value can typically be done efficiently. There are three IPID assignment algorithms: sequentially incrementing (the OS increments IPID value by one for every sent packet), per-destination sequentially incrementing (the OS increments IPID by one for every packet sent to a given destination), and random \cite{frag:vulnerable:journal,knockel2014counting}. We describe the three cases below.

\paragraph{Sequentially Incrementing IPID}
Most nameservers use a sequentially incrementing IPID - this is the most efficient algorithm with least overhead on the OS, e,g., Windows OSes use a sequentially incrementing IPID.

The attacker samples the IPID value from the nameserver and samples the IPID increase rate. Then the attacker calculates the IPID value that will be assigned at the time the nameserver sends the DNS response to the victim DNS resolver. The attacker uses this value in the second spoofed fragment. The attacker can also send multiple fragments with different IP ID values to increase his chances to hit the correct IPID value.

\paragraph{Per-Destination IPID} Linux versions are using a per-destination incrementing IPID assignment. The attacker can apply the techniques presented in \cite{knockel2014counting} for predicting the IPID values. 

\paragraph{Random IPID} Very few servers use random IPID values, less than $1\%$. The reason is the overhead that it introduces on the server. Specifically, instead of maintaining a single counter (as in the case of globally incrementing) or one counter per destination (in the case of per destination incrementing IPID), in this case the server has to maintain multiple counters, and to continually check for collisions, i.e., that it does not select an IPID that was already allocated.

The success probability of the attack in case of a single fragment is $\frac{1}{2^{16}}$. The attacker can increase its success probability by sending multiple fragments, each with a different IPID value. Assuming an infinite size defragmentation cache, if the attacker sends $2^{16}$ fragments, its success probability is 1. The existing OSes however limit the number of fragments that can be sent, e.g., Windows to 100 fragments, recent Linux versions to 64 and older allow several thousand fragments \cite{kernel:org}. In Linux, the limit is set via {\em ip\_frag\_max\_dist} parameter. 




\subsection{Constructing Second Fragment}\label{sc:2:frag}
Essentially for many domains of the LIRs the attacker can control even the answer section of a DNS response if fragmentation is at around 200 bytes. Consider fragmentation at 68 bytes. Given a nameserver whose responses fragment so that the first fragment is 68 bytes long, the attacker can control the entire answer section. The headers take 40 bytes: IP header is 20 bytes, UDP header is 8 bytes, DNS header is 12 bytes. The query part (which is the first part in the response) copies the QNAME ($n+1$ bytes, for QNAME of length $n$) together with the CLASS (2 bytes) and type (2 bytes). So a QNAME of length 23 or more bytes results in an {\sf Answer} section getting fragmented before the answer part. Even with first fragment of size 200 bytes, the attacker controls the answer part using QNAME of 160 or more bytes (DNS names can be up to 253 characters). %
In other cases, where fragmentation occurs significantly above 200 bytes, the attacker controls the authority and additional sections.


\subsection{Fragmentation}\label{sc:res:frag} The resolver of the RIR accept fragmented DNS responses. Our attack based on overwriting IP fragments, hence it  applies only if fragmented responses can be received. The measurement study was performed as illustrated in Appendix, Figure \ref{fig:step1_dnsprobe}. In this study we measure if the RIR's resolver receives fragments and also which fragment sizes are supported. All the resolvers were found to accept fragments of all the different sizes that we evaluated - 1280, 576, 296 and 68 bytes (see Table \ref{resolvers_accepting_fragments_table}).

The attacker triggers a DNS request, we do this via an email to the email server of the RIR (Appendix, step (1) in Figure \ref{fig:step1_dnsprobe}). In the {\tt HELO} and {\tt MAIL FROM} SMTP headers we use the domain under our control {\tt attacker.info}. In step (2-4) the DNS resolver (on behalf of the email server) of the RIR requests {\tt MX} and {\tt A} records of attacker's email exchanger. The attacker returns a {\tt CNAME} record. 

Using a {\tt CNAME} record we create a chain of requests which allows us by trigerring only one query to evaluate support of different MTU values (of 1280, 576, 296 and 68 bytes) by the RIR's DNS resolver. Hence, steps (4-6) in Figure \ref{fig:step1_dnsprobe} in Appendix are repeated with different values of MTU in ICMP error message. If our nameserver receives a retransmission of the request from the DNS resolver we know that it does not accept fragments with the most recent MTU value, whereas if we receive an Email from the Email server of the RIR we know that it the resolver of the RIR accepted the most recently provided fragments.

\subsection{BGP and RPKI}\label{sc:bgp}
The Border Gateway Protocol (BGP) computes routes between Autonomous Systems (ASes) - networks which make up the Internet. ASes range from large ISPs and content providers to small businesses and universities. BGP is notoriously vulnerable to devastating attacks and configuration errors. Consequently, nation states and corporations are in constant danger from attacks that utilise BGP's insecurity to disconnect ASes from the Internet and to launch highly effective man-in-the-middle attacks. A particularly worrisome and common attack vector is {\em IP prefix hijacking}, where an AS advertises in BGP an IP prefix not belonging to it. Prefix hijacks are effective and easy to launch, with the extra benefit of a plausible excuse: benign configuration errors~\cite{rpkimisconfig}. Every year several high-profile incidents resulting from prefix hijacks make the news (e.g., ~\cite{renesys_bel_ice,bgpmon:syria,BGPmon_Indosat,BGPmon_turk}), and many others go under the radar~\cite{conf/ndss/VervierTD15}.

The \emph{Resource Public Key Infrastructure (RPKI)}~\rfc{6480} is a hierarchical certification system. RPKI stores {\em Route Origin Authorizations (ROAs)}, signed records that bind an IP address block to the AS that is allowed to advertise it in BGP. ROAs can be leveraged by BGP routers to perform {\em Route-Origin Validation (ROV)}~\rfc{7115}, \rfc{6811}: identifying and discarding ``invalid'' BGP route-advertisements from unauthorised ASes, thus protecting against IP prefix hijacking. Beyond being the leading and, thus far, only standardised solution to prefix hijacking, RPKI is also a prerequisite for prominent routing security mechanisms such as BGPsec~\rfc{8205}, and for other proposals for defending against BGP path-manipulation attacks, e.g.,~\cite{conf/hotnets/CohenGHS15,conf/sigcomm/CohenGHS16,sobgp}.

%


\subsection{Attack Against LIR}\label{ap:sec:lir}
Direct attack against the LIR via DNS cache poisoning is illustrated in Figure \ref{fig:direct:attack}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.42\textwidth]{img/directattack-crop.pdf}
    \caption{Attack against LIR. }
    \label{fig:direct:attack}\label{fig:my_label}
    \vspace{-10pt}
\end{figure}

\subsection{Domain Name System (DNS)}\label{sc:dns:bck}
Domain Name System (DNS), \rfc{1034} and \rfc{1035}, is a distributed database containing mappings for resources (also called {\em resource records (RRs)}), from {\em domain names} to different values. The most popular and widely used mappings, \cite{gao2013empirical}, are for IP addresses, represented by {\tt A} type RRs, that map a domain name to its IPv4 address, and nameservers, represented by {\tt NS} type RRs, that map a domain name to a nameserver. The resource records in DNS correspond to the different services run by the organisations and networks, e.g., hosts, servers, network blocks. DNS packet is illustrated in Figure \ref{fig:dns:format}.
\begin{figure} [h]
  \begin{center}
   \includegraphics[width=0.45\textwidth]{img/pkt_dns_question-crop.pdf}
		\caption{DNS request packet from DNS resolver at 30.0.0.1 to a nameserver at 123.0.0.53}
		\label{fig:dns:format}
  \end{center}
  \vspace{-10pt}
\end{figure}
DNS is a client-server protocol, used by the resolvers to retrieve RRs stored in the zone files maintained by the nameservers. The resolvers communicate to the nameservers using a simple request-response protocol (typically over UDP); for instance, (abstracting out details) to translate {\tt www.foo.bar} resolvers locate the nameserver {\tt ns.foo.bar}, authoritative for {\tt foo.bar}, and obtain the IP address of the machine hosting the web server of the website {\tt www.foo.bar}. Resolvers store the DNS records, returned in responses, in their caches for the duration indicated in the Time To Live (TTL) field of each record set.

The zones are structured hierarchically, with the root zone at the first level, Top Level Domains (TLDs) at the second level, and millions of Second Level Domains (SLDs) at the third level. The IP addresses of the 13 root servers are provided via the {\em hints} file, or compiled into DNS resolvers software and when a resolver's cache is empty, every resolution process starts at the root. According to the query in the DNS request, the root nameserver redirects the resolver, via a {\tt referral} response type, to a corresponding TLD, under which the requested resource is located. There are a number of TLDs types, most notably: {\em country code TLD} (ccTLD), which domains are (typically) assigned to countries, e.g., {\tt us, il, de}, and {\em generic TLD} (gTLD), whose domains are used by organisations, e.g., {\tt com, org}, and also by US government and military, e.g., {\tt gov, mil}. Domains in SLDs can also be used to further delegate subdomains to other entities, or can be directly managed by the organisations, e.g., as in the case of {\tt ibm.com, google.com}.


\subsection{Domain Name System Security Extensions (DNSSEC)}\label{sc:dnssec:bck}
\widowpenalty0
\clubpenalty0

To mitigate the DNS cache poisoning attacks, the IETF designed and standardised Domain Name System Security Extensions (DNSSEC)~\rfc{4033} to \rfc{4035}. Unfortunately DNSSEC requires significant changes to the DNS infrastructure as well as to the protocol, and although proposed and standardised already in 1997, it is still not widely deployed. The low adoption of DNSSEC in tandem with the recent wave of cache poisoning vulnerabilities and evidence for DNS injections in the Internet stimulated efforts within the operational and research communities to standardise alternative {\em easy to adopt} defences.

Recently vulnerabilities and misconfigurations were found in DNSSEC keys generation and management procedures exposing a large fraction of signed domains (more than $35\%$) to attacks, \cite{dai2016dnssec,shulman2017one,chung2017longitudinal}. Furthermore, as \cite{hao2018end} showed DNSSEC does not prevent attacks which replay DNSSEC-signed DNS response to redirect clients to incorrect servers in Content Distribution Networks (CDNs).

We show how to evaluate if a DNS resolver correctly validates DNSSEC in Figure \ref{fig:step1_dnssec}.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.40\textwidth]{img/step1_dnssec-crop.pdf}
    \caption{(Step 1.2 Figure \ref{fig:sequence_overview}) Probing the RIR's DNS resolver for DNSSEC validation.}
    \label{fig:step1_dnssec}
\end{figure}


\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.40\textwidth]{img/step4-crop.pdf}
    \caption{(Step 4 in Figure \ref{fig:sequence_overview}) Triggering the password recovery E-mail and obtain target LIR account data.}
    \label{fig:step4_pwrest}
    \vspace{-5pt}
\end{figure}

\begin{table}[ht!]
\begin{center}
\small
\begin{tabular}{ | P{1.4cm} | P{1.1cm} | P{1.2cm} | P{0.8cm} | P{1cm} | P{0.8cm} |}
    \hline
    RIR & Iteration-1$^{st}$ & -2$^{nd}$ & -3$^{rd}$ & -4$^{th}$ & -5$^{th}$ \\
    \hline
    AFRINIC & 0.10 & 0.08 & 0.07 & 0.08 & 0.26 \\ 
    APNIC & 452.57 & 144.21 & 566.88 & 474.01 & 391.11 \\ 
    ARIN & 3.27 & 1.72 & 2.89 & 2.81 & 1.56 \\
    LACNIC & 0.91 & 0.32 & 0.41 & 0.34 & 0.32 \\ 
    RIPE NCC & 0.33 & 0.15 & 0.23 & 0.19 & 0.16 \\ \hline
\end{tabular}
\end{center}
\caption{Latency (in seconds) between E-mail Registration and Resolver Query. }
\label{latency_table}
\vspace{-5pt}
\end{table}

\begin{table}[!ht]
    \centering
    \footnotesize
    \begin{tabular}{|c|r|r<{\hspace{-6pt}}r|r<{\hspace{-6pt}}r|r<{\hspace{-10pt}}r|}
\hline
RIR         &
\makecell{ \# Tested } \hspace{-5pt} &
\multicolumn{2}{c|}{ \hspace{-5pt} \makecell{ \# Accepting \\ fragments} \hspace{-5pt} }  &
\multicolumn{2}{c|}{ \hspace{-5pt} \makecell{ \# DNSSEC \\ DO set} \hspace{-5pt} }  & 
\multicolumn{2}{c|}{ \hspace{-5pt} \makecell{ \# Vulnerable* } \hspace{-5pt} } \\
\hline
AFRINIC	    & 226	    & 171  &75.6\% & 200  &88.5\% & 19  &8.4\%    \\ %
APNIC	    & 966	    & 395  &40.9\% & 774  &80.1\% & 60  &6.2\%    \\ %
ARIN	    & 1436      & 757  &52.7\% & 1105 &76.9\% & 142 &9.9\%    \\ %
LACNIC	    & 95	    & 43   &45.3\% & 62   &65.3\% & 8   &8.4\%    \\ %
RIPE        & 3271	    & 1479 &45.2\% & 2649 &81.0\% & 235 &7.2\%    \\ %
\hline
All	        & 5994	    & 2845 &47.5\% & 4790 &79.9\% & 464 &7.7\%    \\ %
\hline

    \end{tabular}
    \caption{Measurement study of potential victim LIR resolvers used by their MX mail servers. *Vulnerable = accepting fragments \&\& !DNSSEC DO }
    \label{tab:victim_resolvers}
    \vspace{-15pt}
\end{table}
